Narrowband searches for continuous and long-duration transient gravitational waves from known pulsars in the LIGO-Virgo third observing run

Isolated neutron stars that are asymmetric with respect to their spin axis are possible sources of detectable continuous gravitational waves. This paper presents a fully-coherent search for such signals from eighteen pulsars in data from LIGO and Virgo's third observing run (O3). For known pulsars, efficient and sensitive matched-filter searches can be carried out if one assumes the gravitational radiation is phase-locked to the electromagnetic emission. In the search presented here, we relax this assumption and allow the frequency and frequency time-derivative of the gravitational waves to vary in a small range around those inferred from electromagnetic observations. We find no evidence for continuous gravitational waves, and set upper limits on the strain amplitude for each target. These limits are more constraining for seven of the targets than the spin-down limit defined by ascribing all rotational energy loss to gravitational radiation. In an additional search we look in O3 data for long-duration (hours-months) transient gravitational waves in the aftermath of pulsar glitches for six targets with a total of nine glitches. We report two marginal outliers from this search, but find no clear evidence for such emission either. The resulting duration-dependent strain upper limits do not surpass indirect energy constraints for any of these targets.

==> P2000488_v7.tex <==
This material is based upon work supported by NSF’s LIGO Laboratory which is a major facility
fully funded by the National Science Foundation.
The authors also gratefully acknowledge the support of
the Science and Technology Facilities Council (STFC) of the
United Kingdom, the Max-Planck-Society (MPS), and the State of
Niedersachsen/Germany for support of the construction of Advanced LIGO 
and construction and operation of the GEO600 detector. 
Additional support for Advanced LIGO was provided by the Australian Research Council.
The authors gratefully acknowledge the Italian Istituto Nazionale di Fisica Nucleare (INFN),  
the French Centre National de la Recherche Scientifique (CNRS) and
the Netherlands Organization for Scientific Research, 
for the construction and operation of the Virgo detector
and the creation and support  of the EGO consortium. 
The authors also gratefully acknowledge research support from these agencies as well as by 
the Council of Scientific and Industrial Research of India, 
the Department of Science and Technology, India,
the Science \& Engineering Research Board (SERB), India,
the Ministry of Human Resource Development, India,
the Spanish Agencia Estatal de Investigaci\'on,
the Vicepresid\`encia i Conselleria d'Innovaci\'o, Recerca i Turisme and the Conselleria d'Educaci\'o i Universitat del Govern de les Illes Balears,
the Conselleria d'Innovaci\'o, Universitats, Ci\`encia i Societat Digital de la Generalitat Valenciana and
the CERCA Programme Generalitat de Catalunya, Spain,
the National Science Centre of Poland and the Foundation for Polish Science (FNP),
the Swiss National Science Foundation (SNSF),
the Russian Foundation for Basic Research, 
the Russian Science Foundation,
the European Commission,
the European Regional Development Funds (ERDF),
the Royal Society, 
the Scottish Funding Council, 
the Scottish Universities Physics Alliance, 
the Hungarian Scientific Research Fund (OTKA),
the French Lyon Institute of Origins (LIO),
the Belgian Fonds de la Recherche Scientifique (FRS-FNRS), 
Actions de Recherche Concertées (ARC) and
Fonds Wetenschappelijk Onderzoek – Vlaanderen (FWO), Belgium,
the Paris \^{I}le-de-France Region, 
the National Research, Development and Innovation Office Hungary (NKFIH), 
the National Research Foundation of Korea,
the Natural Science and Engineering Research Council Canada,
Canadian Foundation for Innovation (CFI),
the Brazilian Ministry of Science, Technology, and Innovations,
the International Center for Theoretical Physics South American Institute for Fundamental Research (ICTP-SAIFR), 
the Research Grants Council of Hong Kong,
the National Natural Science Foundation of China (NSFC),
the Leverhulme Trust, 
the Research Corporation, 
the Ministry of Science and Technology (MOST), Taiwan,
the United States Department of Energy,
and
the Kavli Foundation.
The authors gratefully acknowledge the support of the NSF, STFC, INFN and CNRS for provision of computational resources.
% updated June 2021
This work was supported by MEXT, JSPS Leading-edge Research Infrastructure Program, JSPS Grant-in-Aid for Specially Promoted Research 26000005(Kajita 2014-2018), JSPS Grant-in-Aid for Scientific Research on Innovative Areas 2905: JP17H06358, JP17H06361 and JP17H06364, JSPS Core-to-Core Program A. Advanced Research Networks, JSPS Grant-in-Aid for Scientific Research (S) 17H06133 and 20H05639 , JSPS Grant-in-Aid for Transformative Research Areas (A) 20A203: JP20H05854, the joint research program of the Institute for Cosmic Ray Research, University of Tokyo, National Research Foundation (NRF) and Computing Infrastructure Project of KISTI-GSDC in Korea, Academia Sinica (AS), AS Grid Center (ASGC) and the Ministry of Science and Technology (MoST) in Taiwan under grants including AS-CDA-105-M06, Advanced Technology Center (ATC) of NAOJ, Mechanical Engineering Center of KEK.
% \fi
% 
% \ifcoreonly\else
% {\bf For certain collaboration papers, it may be appropriate to acknowledge specific analysis software.
% One template to consider is that used for the GW190425 discovery paper, for which the latex can be
% found here:}\\
% {\small https://git.ligo.org/publications/gw190425/gw190425-discovery/-/blob/master/gw190425-discovery.tex\#L259.}
% \fi
% 
% \ifcoreonly\else
% {\bf For collaboration papers released after March 2020, it may be appropriate to add the following special acknowledgement, BUT the journal may reject it (PRL rejected it). If one chooses, one can include such acknowledgements in arXiv/DCC versions only in that case:}\\
% \fi
% \ifcoreonly\else
% {\it We would like to thank all of the essential workers who put their health at risk during the COVID-19 pandemic, without whom we would not have been able to complete this work.}
% \fi
% 

==> cw_search_setup_table.tex <==
\begin{rotatetable*}
\begin{deluxetable*}{lllccccccccccc}
\tablecaption{
\label{tab:search_setup_parameter}
Set-up parameters for fully coherent \cw search pipelines.
}
\tablehead{\colhead{Name} & \colhead{R.A.} & \colhead{DEC.} & \colhead{$\fgw$} & \colhead{$\Delta\fgw$ (5v)} & \colhead{$\Delta\fgw\,(\F)$} & \colhead{$\fdot$} & \colhead{$\Delta\fdot$ (5v)} &
\colhead{$\Delta\fdot\,(\F)$} &
\colhead{$\fddot$} &
\colhead{$\Delta\fddot$}&
\colhead{$n_{\rm total}^{\rm{5v}}$} & \colhead{$n_{\rm total}^{\F}$} & Ref. \\
\colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{$\times 10^{-13}$} & \colhead{$\times 10^{-15}$} & \colhead{$\times 10^{-15}$} & \colhead{$\times 10^{-23}$} & \colhead{$\times 10^{-23}$} & \colhead{$\times 10^{7}$} & \colhead{$\times 10^7$} &\\
\colhead{} & \colhead{} & \colhead{} & \colhead{Hz} & \colhead{Hz} & \colhead{Hz} & \colhead{$\rm{Hz~s^{-1}}$} & \colhead{$\rm{Hz~s^{-1}}$} & \colhead{$\rm{Hz~s^{-1}}$} & \colhead{$\rm{Hz~s^{-2}}$} & \colhead{$\rm{Hz~s^{-2}}$} & \colhead{} & \colhead{} &
}
\startdata
   J0534+2200\textrm{ bg} &$ 05^{\textrm{h}}34^{\textrm{m}}31.97^{\textrm{s}} $&$  +22^\circ00'52.07'' $&$   59.241 $&$ \ldots $&$  0.24 $&$  -7370.0 $&$    \ldots $&$   2900.0 $&$ 2360.0 $&$     5.2 $&$     \ldots$ &$     983.7 $&a\\
   J0534+2200\textrm{ ag} &$ 05^{\textrm{h}}34^{\textrm{m}}31.97^{\textrm{s}} $&$  +22^\circ00'52.07'' $&$   59.241 $&$   0.24 $&$  0.24 $&$  -7370.0 $&$    2300.0 $&$   2900.0 $&$ 2360.0 $&$     5.2 $&$      498.0$ &$    9362.0 $    &a\\
               J0711--6830 &$ 07^{\textrm{h}}11^{\textrm{m}}54.18^{\textrm{s}} $&$ -68^\circ30'47.37''  $&$  364.234 $&$   0.72 $&$   1.5 $&$ -0.00989 $&$       2.1 $&$    0.004 $&$    0.0 $&$     0.0 $&$      4.391$ &$     45.85 $   &b\\
               J0835--4510 &$ 08^{\textrm{h}}35^{\textrm{m}}20.52^{\textrm{s}} $&$ -45^\circ10'34.28''  $&$   22.371 $&$  0.089 $&$ 0.089 $&$   -313.0 $&$     130.0 $&$    120.0 $&$  504.0 $&$     0.0 $&$       32.9$ &$     281.6 $   &c\\
               J1101--6101 &$ 11^{\textrm{h}}01^{\textrm{m}}44.96^{\textrm{s}} $&$  -61^\circ01'39.6''  $&$   31.846 $&$   0.13 $&$  0.13 $&$    -45.3 $&$      19.0 $&$     18.0 $&$    0.0 $&$     0.0 $&$      7.026$ &$     61.52 $   &d\\
               J1105--6107 &$ 11^{\textrm{h}}05^{\textrm{m}}25.71^{\textrm{s}} $&$ -61^\circ07'55.63'' $&$   31.644 $&$   \ldots $&$  0.13 $&$    -79.7 $&$   \ldots $&$     32.0 $&$  554.0 $&$     35.0 $&$    \ldots $&$     266.0 $& e \\
               J1809--1917 &$ 18^{\textrm{h}}09^{\textrm{m}}43.13^{\textrm{s}} $&$  -19^\circ17'38.2''  $&$   24.166 $&$  0.097 $&$ 0.097 $&$    -74.4 $&$      32.0 $&$     30.0 $&$    3.7 $&$    0.14 $&$      8.886$ &$     152.3 $   &a\\
   J1813-1749\textrm{ bg} &$ 18^{\textrm{h}}13^{\textrm{m}}35.11^{\textrm{s}} $&$ -17^\circ49'57.57''  $&$   44.703 $&$ \ldots $&$  0.18 $&$  -1290.0 $&$    \ldots $&$    510.0 $&$    0.0 $&$     0.0 $&$     \ldots$ &$     92.08 $ &d\\
 J1813-1749\textrm{ full} &$ 18^{\textrm{h}}13^{\textrm{m}}35.11^{\textrm{s}} $&$ -17^\circ49'57.57''  $&$   44.703 $&$   0.18 $&$  0.18 $&$  -1290.0 $&$     520.0 $&$    510.0 $&$    0.0 $&$     0.0 $&$      266.4$ &$    2270.0 $   &d\\
               J1828--1101 &$ 18^{\textrm{h}}28^{\textrm{m}}18.85^{\textrm{s}} $&$ -11^\circ01'51.72''  $&$   27.754 $&$   0.11 $&$  0.11 $&$    -57.0 $&$      23.0 $&$     23.0 $&$   4.23 $&$     9.4 $&$      7.481$ &$    1162.0 $   &a\\
               J1833--0827 &$ 18^{\textrm{h}}33^{\textrm{m}}40.26^{\textrm{s}} $&$ -08^\circ27'31.53''  $&$   23.449 $&$  0.094 $&$ 0.094 $&$    -25.2 $&$      11.0 $&$     10.0 $&$ -0.463 $&$   0.082 $&$      2.873$ &$     242.2 $   &e\\
               J1838--0655 &$  18^{\textrm{h}}38^{\textrm{m}}3.13^{\textrm{s}} $&$  -06^\circ55'33.4''  $&$   28.363 $&$   0.11 $&$  0.11 $&$   -199.0 $&$      83.0 $&$     80.0 $&$   67.1 $&$     7.8 $&$      27.13$ &$     555.4 $   &d\\
               J1856+0245 &$ 18^{\textrm{h}}56^{\textrm{m}}50.91^{\textrm{s}} $&$ +02^\circ45'53.17''  $&$   24.714 $&$  0.099 $&$\ldots $&$   -189.0 $&$      79.0 $&$   \ldots $&$    0.0 $&$     0.0 $&$      22.42$ &$    \ldots $   &a\\
               J1913+1011 &$ 19^{\textrm{h}}13^{\textrm{m}}20.34^{\textrm{s}} $&$ +10^\circ11'22.97''  $&$   55.694 $&$   0.22 $&$  0.22 $&$    -52.5 $&$      23.0 $&$     21.0 $&$ -0.321 $&$     2.6 $&$      15.02$ &$    1951.0 $   &a\\
               J1925+1720 &$ 19^{\textrm{h}}25^{\textrm{m}}27.06^{\textrm{s}} $&$ +17^\circ20'27.42''  $&$   26.434 $&$   0.11 $&$  0.11 $&$    -36.6 $&$      15.0 $&$     15.0 $&$   3.93 $&$     6.3 $&$      4.538$ &$     469.2 $   &a\\
               J1928+1746 &$ 19^{\textrm{h}}28^{\textrm{m}}42.55^{\textrm{s}} $&$ +17^\circ46'29.67''  $&$   29.097 $&$   0.12 $&$  0.12 $&$    -55.7 $&$      23.0 $&$     22.0 $&$    0.0 $&$     0.0 $&$      7.845$ &$     68.41 $   &a\\
               J1935+2025 &$ 19^{\textrm{h}}35^{\textrm{m}}41.94^{\textrm{s}} $&$  +20^\circ25'40.1''  $&$   24.955 $&$  0.092 $&$   0.1 $&$   -189.0 $&$      79.0 $&$     76.0 $&$   95.0 $&$     3.4 $&$      20.99$ &$     581.3 $   &a\\
               J1952+3252 &$ 19^{\textrm{h}}52^{\textrm{m}}58.21^{\textrm{s}} $&$ +32^\circ52'40.51''  $&$   50.587 $&$    0.2 $&$   0.2 $&$    -74.9 $&$      32.0 $&$     30.0 $&$   2.92 $&$   0.012 $&$      18.61$ &$    3908.0 $   &f\\
               J2124--3358 &$ 21^{\textrm{h}}24^{\textrm{m}}43.84^{\textrm{s}} $&$ -33^\circ58'45.06''  $&$  405.588 $&$   0.91 $&$   1.6 $&$  -0.0169 $&$       2.1 $&$   0.0068 $&$    0.0 $&$     0.0 $&$      5.595$ &$     48.06 $   &g\\
               J2229+6114 &$  22^{\textrm{h}}29^{\textrm{m}}6.57^{\textrm{s}} $&$  +61^\circ14'10.9''  $&$   38.709 $&$   0.15 $&$  0.16 $&$   -590.0 $&$     240.0 $&$    260.0 $&$ 1170.0 $&$     0.0 $&$      107.3$ &$    1021.0 $   &f
\enddata
\tablecomments{
 This table lists frequency $\fgw$ and spin-down ($\fdot$,$\fddot$) parameters corresponding to twice
 the rotational parameters in the pulsar ephemerides at the start of the O3 run
 (2019 April 1 15:00 UTC, MJD 58574.000),
 as discussed in Sec.~\ref{sec:signal}.
 Right ascension (RA) and Declination (DEC) are given in J2000 coordinates.
 In the column headings,
 $\F$ stands for the $\F$-statistic search discussed in Sec.~\ref{sec:fstat-method}
 and $5$v stands for the 5$n$-vector method discussed in Sec.~\ref{sec:fivevec-method}.
 The suffixes ``bg'' and ``ag'' refer to ``before'' and ``after'' glitch respectively, while ``full'' corresponds to the full run in the case of \psr{1813--1749}. \\
(a) Jodrell Bank 42ft telescope and Lovell telescope
(b) MeerKAT telescope (part of the MeerTime project) \citep{MeerKAT_reference}
(c) University of Tasmania's Mt. Pleasant Observatory 26m telescope
(d) \ac{nicer}~\citep{NICER_reference}
(e) \ac{most}~\citep{UTMOST_reference,Jankowski2018abc,Lower:2020mjq}
(f) \ac{chime}~\citep[part of the \ac{chime} pulsar project,][]{CHIME_reference,Amiri_2021}
(g) Nan\c{c}ay Decimetric Radio Telescope}
\end{deluxetable*}
\end{rotatetable*}

==> cw_search_upper_limits_table.tex <==
\begin{deluxetable*}{lccccccccccc}
\tablecaption{
 \ul results on \cw strain from the 5$n$-vector (5v) and \Fstat ($\F$) pipelines.
 \label{tab:upper_limits_results_tab}
}
\tablehead{\colhead{Name} & \colhead{$f$} & \colhead{$h_0^{95}$ (5v)} & \colhead{$h_0^{95}$ ($\F$)} & \colhead{$h_{\rm sd}$} & \colhead{$h_0^{95} / h_{\rm sd}$} & \colhead{$h_0^{95} / h_{\rm sd}$} & \colhead{$\epsilon$ (5v)} & \colhead{$\epsilon$ ($\F$)} & \colhead{$\epsilon_{\rm sd}$} & \colhead{$d$} & \colhead{$\sigma_d$} \\
\colhead{} & \colhead{Hz} & \colhead{$\times10^{-26}$} & \colhead{$\times10^{-26}$} & \colhead{$\times10^{-26}$}& \colhead{(5v)}& \colhead{ ($\F$)}& \colhead{$\times10^{-5}$}& \colhead{$\times10^{-5}$}& \colhead{$\times10^{-5}$}& \colhead{kpc} &\colhead{kpc}}
\startdata
J0534+2200 bg   & 59.24  & ...  & 8.79  & 143.0  & ...   & 0.061  & ...    & 4.6    & 76.0    & 2.00$\;^{a}$ & 0.5 \\
J0534+2200 ag   & 59.24  & 5.2  & 6.09  & 143.0  & 0.036 & 0.043  & 2.7    & 3.2    & 76.0    & 2.00$\;^{a}$ & 0.5 \\
J0711--6830      & 364.23 & 2.29 & 2.69  & 1.25   & 1.8   & 2.2    & 0.0017 & 0.002  & 0.00095 & 0.11 & 0.041 \\
J0835--4510      & 22.37  & 36.2 & 39.5  & 341.0  & 0.11  & 0.12   & 19.0   & 21.0   & 180.0   & 0.28$\;^{b}$ & 0.02 \\
J1101--6101      & 31.85  & 8.96 & 10.5  & 4.25   & 2.1   & 2.5    & 59.0   & 68.0   & 28.0    & 7.00 & 2.7 \\
J1105--6107      & 31.64  & ...\tablenotemark{$\dagger$} & 10.1  & 17.1   & ...  & 0.59   & ...   & 23.0   & 38.0    & 2.36 & 0.92 \\
J1809--1917      & 24.17  & 21.7 & 26.1  & 13.7   & 1.6   & 1.9    & 110.0  & 140.0  & 73.0    & 3.27 & 1.3 \\
J1813--1749 full & 44.70  & 4.61 & 5.85  & 21.9   & 0.21  & 0.27   & 10.0   & 13.0   & 64.0    & 6.20$\;^{c}$ & 2.4 \\
J1813--1749 bg   & 44.70  & ...  & 9.61  & 21.9   & ...   & 0.44   & ...    & 21.0   & 64.0    & 6.20$\;^{c}$ & 2.4 \\
J1828--1101      & 27.75  & 14.8 & 16.3  & 7.67   & 1.9   & 2.1    & 87.0   & 96.0   & 45.0    & 4.77 & 1.9 \\
J1833--0827      & 23.45  & 22.9 & 29.3  & 5.88   & 3.9   & 5.0    & 180.0  & 230.0  & 46.0    & 4.50 & 1.8 \\
J1838--0655      & 28.36  & 13.2 & 15.3  & 10.2   & 1.3   & 1.5    & 100.0  & 120.0  & 79.0    & 6.60$\;^{d}$ & 0.9 \\
J1856+0245      & 19.35  & 20.5 & ...   & 11.2   & 1.8   & ...    & 200.0  & ...    & 110.0   & 6.32 & 2.46 \\
J1913+1011      & 55.69  & 3.47 & 4.37  & 5.36   & 0.65  & 0.81   & 4.9    & 6.1    & 7.5     & 4.61 & 1.8 \\
J1925+1720      & 26.43  & 14.3 & 17.6  & 5.93   & 2.4   & 3.0    & 98.0   & 120.0  & 41.0    & 5.06 & 2.0 \\
J1928+1746      & 29.10  & 10.5 & 13.5  & 8.15   & 1.3   & 1.7    & 51.0   & 66.0   & 39.0    & 4.34 & 1.7 \\
J1935+2025      & 24.95  & 19.2 & 23.7  & 15.3   & 1.3   & 1.5    & 130.0  & 170.0  & 110.0   & 4.60 & 1.8 \\
J1952+3252      & 50.59  & 3.73 & 4.93  & 10.3   & 0.36  & 0.48   & 4.1    & 5.5    & 11.0    & 3.00$\;^{e}$ & 2.0 \\
J2124--3358      & 405.59 & 2.4  & 2.9   & 0.374  & 6.4   & 7.7    & 0.0057 & 0.0068 & 0.00095 & 0.44$\;^{f}$ & 0.05 \\
J2229+6114      & 38.71  & 5.78 & 7.23  & 33.1   & 0.17  & 0.22   & 11.0   & 14.0   & 63.0    & 3.00$\;^{g}$ & 2.0
\enddata
\tablecomments{
We show the \uls on strain amplitude at 95\% confidence for both pipelines, $h_0^{95}$, the spin-down limit for each target $h_{\rm sd}$ along with the implied limit on ellipticity $\epsilon$ for each pipeline, and the limit on ellipticity implied by the spin-down limit $\epsilon_{\rm sd}$.
Finally, we also show the ratio of the 95\% confidence \ul and the spin-down limit.
We surpass the spin-down limit for \numnarrowbandexceedspindwon targets:  \psr{0534+2200}, \psr{0835-4510}, \psr{1105--6107}, \psr{1813--1749}, \psr{1913+1011}, \psr{1952+3252}, and \psr{2229+6115}.
We do not show uncertainty on \uls here, although we discuss uncertainty due to the \ul-setting method as well as calibration uncertainty in Sec.~\ref{sec:conclusion}.
Distance estimates $d$ and their uncertainties $\sigma_d$ are from dispersion measures \citep[with a fiducial uncertainty of 40\% from][]{2017ApJ...835...29Y} unless noted with one of the following: (a)~\citet{Kaplan:2008qm} (b)~\citet{2003ApJ...596.1137D} (c)~\citet{CamiloRansom2021} (d)~\citet{GotthelfHalpern2008} (e)~\citet{2012ApJ...755...39V} (f)~\citet{ReardonShannon2021} (g)~\citet{HalpernCamilo2001}.
}
\tablenotetext{\dagger}{Due to technical issues, the 5$n$-vector analysis for \psr{1105--6107} was not completed in time for this paper.}
\end{deluxetable*}
